Ba$^{2+}$ ion trapping by organic submonolayer: towards an ultra-low background neutrinoless double beta decay detector

If neutrinos are their own antiparticles, the otherwise-forbidden nuclear reaction known as neutrinoless double beta decay ($\beta\beta 0\nu$) can occur, with a characteristic lifetime which is expected to be very long, making the suppression of backgrounds a daunting task. It has been shown that detecting (``tagging'') the Ba$^{+2}$ dication produced in the double beta decay ${}^{136}\mathrm{Xe} \rightarrow {}^{136}$Ba$^{+2}+ 2 e + (2 \nu)$ in a high pressure gas experiment, could lead to a virtually background free experiment. To identify these \Bapp, chemical sensors are being explored as a key tool by the NEXT collaboration . Although used in many fields, the application of such chemosensors to the field of particle physics is totally novel and requires experimental demonstration of their suitability in the ultra-dry environment of a xenon gas chamber. Here we use a combination of complementary surface science techniques to unambiguously show that Ba$^{+2}$ ions can be trapped (chelated) in vacuum by an organic molecule, the so-called fluorescent bicolour indicator (FBI) (one of the chemosensors developed by NEXT), immobilized on a surface. We unravel the ion capture mechanism once the molecules are immobilised on Au(111) surface and explain the origin of the emission fluorescence shift associated to the trapping of different ions. Moreover, we prove that chelation also takes place on a technologically relevant substrate, as such, demonstrating the feasibility of using FBI indicators as building blocks of a Ba$^{+2}$ detector.

==> NEXT_collaboration.tex <==
\author[2]{C.~Adams,}
%
\author[11]{H.~Almaz\'an,}
%
\author[26]{V.~\'Alvarez,}
%
\author[24]{B.~Aparicio,}
%
\author[22]{A.I.~Aranburu,}
%
\author[7]{L.~Arazi,}
%
\author[20]{I.J.~Arnquist,}
%
\author[16]{S.~Ayet,}
%
\author[5]{C.D.R.~Azevedo,}
%
\author[2]{K.~Bailey,}
%
\author[26]{F.~Ballester,}
%
\author[21]{J.M.~Benlloch-Rodr\'{i}guez,}
%
\author[14]{F.I.G.M.~Borges,}
%
\author[11]{S.~Bounasser,}
%
\author[3]{N.~Byrnes,}
%
\author[19]{S.~C\'arcel,}
%
\author[19]{J.V.~Carri\'on,}
%
\author[27]{S.~Cebri\'an,}
%
\author[20]{E.~Church,}
%
\author[14]{C.A.N.~Conde,}
%
\author[11]{T.~Contreras,}
%
\author[21,9]{F.P.~Coss\'io,}
%
\author[4]{A.A.~Denisenko,}
%
\author[25]{G.~D\'iaz,}
%
\author[19]{J.~D\'iaz,}
%
\author[16]{T.~Dickel,}
%
\author[14]{J.~Escada,}
%
\author[26]{R.~Esteve,}
%
\author[11]{A.~Fahs,}
%
\author[7]{R.~Felkai,}
%
\author[13]{L.M.P.~Fernandes,}
%
\author[21,9]{P.~Ferrario,}
%
\author[5]{A.L.~Ferreira,}
%
\author[4]{F.W.~Foss,}
%
\author[13]{E.D.C.~Freitas,}
%
\author[22,9]{Z.~Freixa,}
%
\author[21]{J.~Generowicz,}
%
\author[8]{A.~Goldschmidt,}
%
\author[21,9,c]{J.J.~G\'omez-Cadenas\note[c]{ NEXT Co-spokesperson. },}
%
\author[21]{R.~Gonz\'alez,}
%
\author[25]{D.~Gonz\'alez-D\'iaz,}
%
\author[11]{R.~Guenette,}
%
\author[10]{R.M.~Guti\'errez,}
%
\author[11]{J.~Haefner,}
%
\author[2]{K.~Hafidi,}
%
\author[1]{J.~Hauptman,}
%
\author[13]{C.A.O.~Henriques,}
%
\author[25]{J.A.~Hernando~Morata,}
%
\author[21,23]{P.~Herrero-G\'omez,}
%
\author[26]{V.~Herrero,}
%
\author[11]{J.~Ho,}
%
\author[7]{Y.~Ifergan,}
%
\author[3]{B.J.P.~Jones,}
%
\author[25]{M.~Kekic,}
%
\author[18]{L.~Labarga,}
%
\author[3]{A.~Laing,}
%
\author[6]{P.~Lebrun,}
%
\author[11]{D.~Lopez Gutierrez,}
%
\author[26]{N.~L\'opez-March,}
%
\author[10]{M.~Losada,}
%
\author[13]{R.D.P.~Mano,}
%
\author[19]{J.~Mart\'in-Albo,}
%
\author[19]{A.~Mart\'inez,}
%
\author[7]{G.~Mart\'inez-Lema,}
%
\author[21,19]{M.~Mart\'inez-Vara,}
%
\author[3]{A.D.~McDonald,}
%
\author[2]{Z.E.~Meziani,}
%
\author[3]{K.~Mistry,}
%
\author[21,9]{F.~Monrabal,}
%
\author[13]{C.M.B.~Monteiro,}
%
\author[26]{F.J.~Mora,}
%
\author[19]{J.~Mu\~noz Vidal,}
%
\author[3]{K.~Navarro,}
%
\author[19]{P.~Novella,}
%
\author[3,c]{D.R.~Nygren,}
%
\author[21]{E.~Oblak,}
%
\author[21]{M.~Odriozola-Gimeno,}
%
\author[25,19]{B.~Palmeiro,}
%
\author[6]{A.~Para,}
%
\author[12]{J.~P\'erez,}
%
\author[19]{M.~Querol,}
%
\author[3]{A.~Raymond,}
%
\author[7]{A.B.~Redwine,}
%
\author[25]{J.~Renner,}
%
\author[17]{L.~Ripoll,}
%
\author[21,9]{I.~Rivilla,}
%
\author[10]{Y.~Rodr\'iguez Garc\'ia,}
%
\author[26]{J.~Rodr\'iguez,}
%
\author[23]{C.~Rogero,}
%
\author[3]{L.~Rogers,}
%
\author[21,12]{B.~Romeo,}
%
\author[19]{C.~Romo-Luque,}
%
\author[14]{F.P.~Santos,}
%
\author[13]{J.M.F. dos~Santos,}
%
\author[7]{A.~Sim\'on,}
%
\author[19]{M.~Sorel,}
%
\author[11]{C.~Stanford,}
%
\author[13]{J.M.R.~Teixeira,}
%
\author[4]{P.~Thapa,}
%
\author[26]{J.F.~Toledo,}
%
\author[21]{J.~Torrent,}
%
\author[19]{A.~Us\'on,}
%
\author[5]{J.F.C.A.~Veloso,}
%
\author[4]{T.T.~Vuong,}
%
\author[15]{R.~Webb,}
%
\author[7,e]{R.~Weiss-Babai\note[e]{On leave from Soreq Nuclear Research Center, Yavneh, Israel. },}
%
\author[15,f]{J.T.~White\note[f]{Deceased. },}
%
\author[3]{K.~Woodruff,}
%
\author[19]{N.~Yahlali,}
%
%
%
\affil[1]{
Department of Physics and Astronomy, Iowa State University, Ames, IA 50011-3160, USA}
%
\affil[2]{
Argonne National Laboratory, Argonne, IL 60439, USA}
%
\affil[3]{
Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\affil[4]{
Department of Chemistry and Biochemistry, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\affil[5]{
Institute of Nanostructures, Nanomodelling and Nanofabrication (i3N), Universidade de Aveiro, Campus de Santiago, Aveiro, 3810-193, Portugal}
%
\affil[6]{
Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
%
\affil[7]{
Nuclear Engineering Unit, Faculty of Engineering Sciences, Ben-Gurion University of the Negev, P.O.B. 653, Beer-Sheva, 8410501, Israel}
%
\affil[8]{
Lawrence Berkeley National Laboratory (LBNL), 1 Cyclotron Road, Berkeley, CA 94720, USA}
%
\affil[9]{
Ikerbasque (Basque Foundation for Science), Bilbao, E-48009, Spain}
%
\affil[10]{
Centro de Investigaci\'on en Ciencias B\'asicas y Aplicadas, Universidad Antonio Nari\~no, Sede Circunvalar, Carretera 3 Este No.\ 47 A-15, Bogot\'a, Colombia}
%
\affil[11]{
Department of Physics, Harvard University, Cambridge, MA 02138, USA}
%
\affil[12]{
Laboratorio Subterr\'aneo de Canfranc, Paseo de los Ayerbe s/n, Canfranc Estaci\'on, E-22880, Spain}
%
\affil[13]{
LIBPhys, Physics Department, University of Coimbra, Rua Larga, Coimbra, 3004-516, Portugal}
def MakeArXivAuthorList():
    authorlist=str("NEXT Collaboration: ")
    for a in OrderOfAuthors[:-1]:
        entry=dat.loc[a]
        authorlist+=entry.Initial.strip()+" "+entry.LastName.strip()+", "
    entry=dat.loc[OrderOfAuthors[-1]]
    authorlist=authorlist[:-2]+" and " + entry.Initial.strip()+" "+entry.LastName.strip()
    return authorlist
\affil[14]{
LIP, Department of Physics, University of Coimbra, Coimbra, 3004-516, Portugal}
%
\affil[15]{
Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843-4242, USA}
%
\affil[16]{
II. Physikalisches Institut, Justus-Liebig-Universitat Giessen, Giessen, Germany}
%
\affil[17]{
Escola Polit\`ecnica Superior, Universitat de Girona, Av.~Montilivi, s/n, Girona, E-17071, Spain}
%
\affil[18]{
Departamento de F\'isica Te\'orica, Universidad Aut\'onoma de Madrid, Campus de Cantoblanco, Madrid, E-28049, Spain}
%
\affil[19]{
Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\affil[20]{
Pacific Northwest National Laboratory (PNNL), Richland, WA 99352, USA}
%
\affil[21]{
Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%
\affil[22]{
Department of Applied Chemistry, Universidad del Pais Vasco (UPV/EHU), Manuel de Lardizabal 3, San Sebasti\'an / Donostia, E-20018, Spain}
%
\affil[23]{
Centro de F\'isica de Materiales (CFM), CSIC \& Universidad del Pais Vasco (UPV/EHU), Manuel de Lardizabal 5, San Sebasti\'an / Donostia, E-20018, Spain}
%
\affil[24]{
Department of Organic Chemistry I, University of the Basque Country (UPV/EHU), Centro de Innovaci\'on en Qu\'imica Avanzada (ORFEO-CINQA), San Sebasti\'an / Donostia, E-20018, Spain}
%
\affil[25]{
Instituto Gallego de F\'isica de Altas Energ\'ias, Univ.\ de Santiago de Compostela, Campus sur, R\'ua Xos\'e Mar\'ia Su\'arez N\'u\~nez, s/n, Santiago de Compostela, E-15782, Spain}
%
\affil[26]{
Instituto de Instrumentaci\'on para Imagen Molecular (I3M), Centro Mixto CSIC - Universitat Polit\`ecnica de Val\`encia, Camino de Vera s/n, Valencia, E-46022, Spain}
%
\affil[27]{
Centro de Astropart\'iculas y F\'isica de Altas Energ\'ias (CAPA), Universidad de Zaragoza, Calle Pedro Cerbuna, 12, Zaragoza, E-50009, Spain}
%


==> NEXT_tex <==
C. Adams,$^1$ H. Almazán,$^2$ V. \’Alvarez,$^3$ L. Arazi,$^4$$ I.J. Arnquist,$^5$ S. Ayet,$^6$ C.D.R. Azevedo,$^7$ K. Bailey,$^1$
F. Ballester,$^3$ J.M. Benlloch$-$Rodr\’iguez,$^8$ F.I.G.M. Borges,$^9$ S. Bounasser,$^2$ N. Byrnes,$^{10}$ S. C\’arcel,$^ {11}$ J.V. Carri\’on,$^ {11}$
S. Cebri\’an,$^ {12}$ E. Church,$^5$ C.A.N. Conde,$^9$ T. Contreras,$^2$ A.A. Denisenko,$^ {13}$ G. D\’iaz,$^ {14}$ J. D\’iaz,$^ {11}$ T. Dickel,$^6$
J. Escada,$^9$ R. Esteve,$^3$ A. Fahs,$^2$ R. Felkai,$^4$ L.M.P. Fernandes,$^ {15}$ P. Ferrario,$^{8,16}$ A.L. Ferreira,$^7$ F.W. Foss,$^ {13}$
E.D.C. Freitas,$^ {15}$ J. Generowicz,$^8$ A. Goldschmidt,$^ {17}$ D. Gonz\’alez-D\’iaz,$^ {14}$ R. Guenette,$^2$ R.M. Guti\’errez,$^ {18}$
J. Haefner,$^2$ K. Hafidi,$^1$ J. Hauptman,$^ {19}$ C.A.O. Henriques,$^ {15}$ J.A. Hernando Morata,$^ {14}$ V. Herrero,$^3$ J. Ho,$^2$
Y. Ifergan,$^4$ B.J.P. Jones,$^{10}$ M. Kekic,$^{14}$ L. Labarga,$^ {20}$ A. Laing,$^ {10}$ L. Larizgoitia,$^8$ P. Lebrun,$^ {21}$ D. Lopez
Gutierrez,$^2$ N. L\’opez-March,$^ {11}$ M. Losada,$^ {18}$ R.D.P. Mano,$^ {15}$ J. Mart\’in-Albo,$^ {11}$ A. Mart\’inez,$^ {11}$ G. Mart\’inez-Lema,$^4$
M. Mart\’inez-Vara,$^8$,$^  {11}$ A.D. McDonald,$^ {10}$ Z.E. Meziani,$^1$ K. Mistry,$^{10}$ C.M.B. Monteiro,$^{15}$ F.J. Mora,$^3$
J. Mu\~{n}oz Vidal,$^ {11}$ K. Navarro,$^ {10}$ P. Novella,$^ {11}$ D.R. Nygren,$ {1,∗}$ E. Oblak,$^8$ M. Odriozola-Gimeno,$^8$
B. Palmeiro,$^{14}$,$^{11}$ A. Para,$^{21}$ J. P\’erez,$^{22}$ M. Querol,$^{11}$ A. Raymond,$^{10}$ A.B. Redwine,$^4$ J. Renner,$^{14}$ L. Ripoll,$^{23}$
Y. Rodr\’iguez Garc\’ia,$^{18}$ J. Rodr\’iguez,$^3$ L. Rogers,$^{10}$ B. Romeo,$^8$,$^{22}$ C. Romo-Luque,$^ {11}$ F.P. Santos,$^9$ J.M.F.
dos Santos,$^{15}$ A. Sim\’on,$^4$ M. Sorel,$^{11}$ C. Stanford,$^2$ J.M.R. Teixeira,$^{15}$ P. Thapa,$^{13}$ J.F. Toledo,$^3$ J. Torrent,$^8$
A. Us\’on,$^{11}$ J.F.C.A. Veloso,$^7$ T.T. Vuong,$^{13}$ R. Webb,$^{24}$ J.T. White,$^ {24,†}$ K. Woodruff,$^{10}$ and N. Yahlali$^ {11}$

$^1$Argonne National Laboratory, Argonne, IL 60439, USA
$^2$Department of Physics, Harvard University, Cambridge, MA 02138, USA
$^3$Instituto de Instrumentaci\’on para Imagen Molecular I3M (CSIC-UPV), Valencia, E-46022, Spain
$^4$Unit of Nuclear Engineering, Faculty of Engineering Sciences, Ben-Gurion University of the Negev, Beer-Sheva, 8410501, Israel
$^5$Pacific Northwest National Laboratory (PNNL), Richland, WA 99352, USA
$^6$II. Physikalisches Institut, Justus-Liebig-Universitat Giessen, Giessen, Germany
$^7$Institute of Nanostructures, Nanomodelling and Nanofabrication (i3N), Universidade de Aveiro, Campus de Santiago, Aveiro, 3810-193, Portugal
$^8$Donostia International Physics Center DIPC, San Sebasti\’an / Donostia, E-20018, Spain
$^9$LIP, Department of Physics, University of Coimbra, Coimbra, 3004-516, Portugal
$^{10}$Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA
$^{11}$Instituto de F\’isica Corpuscular (IFIC), CSIC & Universitat de Val`encia, Paterna, E-46980, Spain
$^{12}$Centro de Astropart\’iculas y F\’isica de Altas Energ\’ias (CAPA), Universidad de Zaragoza, Zaragoza, E-50009, Spain
$^{13}$Department of Chemistry and Biochemistry, University of Texas at Arlington, Arlington, TX 76019, USA
$^{14}$Instituto Gallego de F\’isica de Altas Energ\’ias, Univ. de Santiago de Compostela,
Campus sur, Santiago de Compostela, E-15782, Spain
$^{15}$LIBPhys, Physics Department, University of Coimbra, Coimbra, 3004-516, Portugal
$^{16}$Ikerbasque, Basque Foundation for Science, Bilbao, E-48009, Spain
$^{17}$Lawrence Berkeley National Laboratory (LBNL), Berkeley, CA 94720, USA
$^{18}$Centro de Investigaci\’on en Ciencias B\’asicas y Aplicadas, Universidad Antonio Nari ̃no, Sede Circunvalar, Bogot\’a, Colombia
$^{19}$Department of Physics and Astronomy, Iowa State University, Ames, IA 50011-3160, USA
$^{20}$Departamento de F\’isica Te\’orica, Universidad Aut\’onoma de Madrid,
Campus de Cantoblanco, Madrid, E-28049, Spain
$^{21}$Fermi National Accelerator Laboratory, Batavia, IL 60510, USA
$^{22}$Laboratorio Subterr\’aneo de Canfranc, Canfranc Estaci\’on, E-22880, Spain
$^{23}$Escola Polit`ecnica Superior, Universitat de Girona, Girona, E-17071, Spain
$^{24}$Department of Physics and Astronomy, Texas A&M University, College Station, TX 77843-4242, USA
∗ NEXT Co-spokesperson.
† Deceased.


